The Economic Complexity of US Metropolitan Areas

We calculate measures of economic complexity for US metropolitan areas for the years 2007-2015 based on industry employment data. We show that the concept of economic complexity translates well from the cross-country to the regional setting, and is able to incorporate local as well as traded industries. The largest cities and the Northeast of the US have the highest average complexity, while traded industries are more complex than local-serving ones on average, but with some exceptions. On average, regions with higher complexity have a higher income per capita, but those regions also were more affected by the financial crisis. Finally, economic complexity is a significant predictor of within-decreases in income per capita and population. Our findings highlight the importance of subnational regions, and particularly metropolitan areas, as units of economic geography.

==> Figures/MainReg/CrossReg/xc_2015_eci_naics_all_pop_msacnty_bin_lq50.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Tue, Jan 22, 2019 - 11:31:03 PM
\begin{table}[!htbp] \centering 
  \caption{Cross-Section Regression: Population (in 1,000) 2015 (NAICS, $CM_{r,i}$, ECI)} 
  \label{} 
\footnotesize 
\begin{tabular}{@{\extracolsep{5pt}}lccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{5}{c}{\textit{Dependent variable:}} \\ 
\cline{2-6} 
\\[-1.8ex] & \multicolumn{5}{c}{Population (in 1,000) 2015} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5)\\ 
\hline \\[-1.8ex] 
 ECI & 2,281.887$^{***}$ & 1,562.833$^{***}$ & 2,047.848$^{***}$ & 2,311.708$^{***}$ & 1,634.506$^{***}$ \\ 
  & (161.284) & (166.339) & (195.149) & (162.196) & (187.423) \\ 
  & & & & & \\ 
 Unemployment &  & 45.137 &  &  & $-$14.490 \\ 
  &  & (30.251) &  &  & (34.048) \\ 
  & & & & & \\ 
 ManuShare &  & $-$26.407$^{***}$ &  &  & $-$37.967$^{***}$ \\ 
  &  & (8.443) &  &  & (9.398) \\ 
  & & & & & \\ 
 Patent &  & 0.662$^{***}$ &  &  & 0.620$^{***}$ \\ 
  &  & (0.060) &  &  & (0.061) \\ 
  & & & & & \\ 
 Income per Capita &  & $-$22.578$^{***}$ &  &  & $-$14.440$^{*}$ \\ 
  &  & (8.070) &  &  & (8.681) \\ 
  & & & & & \\ 
 MedianAge &  &  & $-$2.241 &  & $-$5.357 \\ 
  &  &  & (14.556) &  & (13.366) \\ 
  & & & & & \\ 
 Education &  &  & $-$21.870$^{**}$ &  & $-$40.344$^{***}$ \\ 
  &  &  & (9.624) &  & (10.711) \\ 
  & & & & & \\ 
 BlackShare &  &  & 18.532$^{**}$ &  & 16.955$^{**}$ \\ 
  &  &  & (8.242) &  & (8.094) \\ 
  & & & & & \\ 
 Foreign &  &  & 69.928$^{***}$ &  & 28.039$^{**}$ \\ 
  &  &  & (11.469) &  & (12.760) \\ 
  & & & & & \\ 
 UnionCoverage &  &  &  & $-$21.545 & 29.285$^{*}$ \\ 
  &  &  &  & (19.478) & (17.233) \\ 
  & & & & & \\ 
 MinimumWage &  &  &  & 143.555 & $-$159.944 \\ 
  &  &  &  & (124.805) & (116.715) \\ 
  & & & & & \\ 
 Vote &  &  &  & $-$29.491$^{***}$ & 8.333 \\ 
  &  &  &  & (9.797) & (8.929) \\ 
  & & & & & \\ 
 Constant & $-$2,333.939$^{***}$ & $-$633.898 & $-$1,932.575$^{***}$ & $-$2,122.547$^{**}$ & 1,301.741 \\ 
  & (225.396) & (497.749) & (682.040) & (914.565) & (940.530) \\ 
  & & & & & \\ 
\hline \\[-1.8ex] 
Observations & 312 & 312 & 312 & 312 & 312 \\ 
R$^{2}$ & 0.392 & 0.592 & 0.478 & 0.411 & 0.628 \\ 
Adjusted R$^{2}$ & 0.390 & 0.586 & 0.470 & 0.403 & 0.613 \\ 
Residual Std. Error & 1,385.809 & 1,142.602 & 1,292.493 & 1,370.994 & 1,104.572 \\ 
F Statistic & 200.172$^{***}$ & 88.894$^{***}$ & 56.100$^{***}$ & 53.564$^{***}$ & 42.003$^{***}$ \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{5}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 

